Brain4Cars: Car That Knows Before You Do via Sensory-Fusion Deep Learning Architecture

Advanced Driver Assistance Systems (ADAS) have made driving safer over the last decade. They prepare vehicles for unsafe road conditions and alert drivers if they perform a dangerous maneuver. However, many accidents are unavoidable because by the time drivers are alerted, it is already too late. Anticipating maneuvers beforehand can alert drivers before they perform the maneuver and also give ADAS more time to avoid or prepare for the danger. In this work we propose a vehicular sensor-rich platform and learning algorithms for maneuver anticipation. For this purpose we equip a car with cameras, Global Positioning System (GPS), and a computing device to capture the driving context from both inside and outside of the car. In order to anticipate maneuvers, we propose a sensory-fusion deep learning architecture which jointly learns to anticipate and fuse multiple sensory streams. Our architecture consists of Recurrent Neural Networks (RNNs) that use Long Short-Term Memory (LSTM) units to capture long temporal dependencies. We propose a novel training procedure which allows the network to predict the future given only a partial temporal context. We introduce a diverse data set with 1180 miles of natural freeway and city driving, and show that we can anticipate maneuvers 3.5 seconds before they occur in real-time with a precision and recall of 90.5\% and 87.4\% respectively.

==> experiment_icra.tex <==
% !TEX root = main.tex

\section{Experiments}
\label{experiments}
We evaluate our proposed architecture on the task of maneuver anticipation~\citep{BoschURBAN,Jain15,Morris11,Tawari14b}. 
This is an important problem because in the US alone 33,000 people die in road accidents every year -- a majority of which are due to dangerous maneuvers. Advanced Driver Assistance Systems (ADAS) have made driving safer by alerting drivers whenever they commit a dangerous maneuver. Unfortunately, many accidents are unavoidable because by the time drivers are alerted it is already too late. Maneuver anticipation can avert many accidents by alerting drivers \textit{before} they perform a dangerous maneuver~\citep{Rueda04}.

We evaluate on the driving data set publicly released by Jain et al.~\citep{Jain15}. The data set consists of 1180 miles of natural freeway and city driving collected from 10 drivers over a period of two months. It contains videos with both inside and outside views of the vehicle, the vehicle's speed, and GPS coordinates. The data set is annotated with 700 events consisting of 274 lane changes, 131 turns, and 295 randomly sampled instances of driving straight. Each lane change and turn is also annotated with the start time of the maneuver, i.e. right before the wheel touches the lane marking or the vehicle yaws at the intersection, respectively. We augment the data set using the technique described in Section~\ref{subsec:augmentation} and generate 2250 events from the 700 original events. We train our deep learning architectures on the augmented data. {We will make our code for data augmentation and maneuver anticipation publicly available at: \url{http://www.brain4cars.com}}

We compare our deep RNN architecture with the following baseline algorithms:
\begin{packed_enum}
\item \textit{Chance:} Uniformly randomly anticipates a maneuver.
\item \textit{Random-forest:} A discriminative classifier that learns an ensemble of 150 decision trees.
\item \textit{SVM~\citep{Morris11}:} Support Vector Machine classifier used by Morris et al.~\citep{Morris11} for maneuver anticipation. 
\item \textit{IOHMM~\citep{Jain15}:} Input-Output Hidden Markov Model~\citep{Bengio95} used by Jain et al.~\citep{Jain15} for maneuver anticipation.  
\item \textit{AIO-HMM~\citep{Jain15}:} This model extends IOHMM by including autoregressive connections in the output layer. AIO-HMM achieved state-of-the-art performance in Jain et al.~\citep{Jain15}. 
\end{packed_enum}

In order to study the effect of our design choices we also compare the following modifications of our architecture:

\begin{packed_enum}
\setcounter{enumi}{5}
\item \textit{Simple-RNN (S-RNN):} In this architecture sensor streams are fused by simple concatenation and then passed through a single RNN with LSTM units. 
\item \textit{Fusion-RNN-Uniform-Loss (F-RNN-UL):} In this architecture sensor streams are passed through separate RNNs, and the high-level representations from RNNs are then fused via a fully-connected layer. The loss at each time step takes the form $-\log(y_t^k)$. 
\item \textit{Fusion-RNN-Exp-Loss (F-RNN-EL):} This architecture is similar to F-RNN-UL, except that the loss exponentially grows with time $-e^{-(T-t)}\log(y_t^k)$. 
\end{packed_enum}

We use the RNN and LSTM implementations provided by Jain~\citep{Neuralmodels}. In our RNNs we use a single layer LSTM of size 64 with sigmoid gate activations and tanh activation for hidden representation. Our fully connected fusion layer uses tanh activation and outputs a 64 dimensional vector. Our overall architecture (F-RNN-EL and F-RNN-UL) have nearly 25,000 parameters that are learned using RMSprop~\citep{Dauphin15}. 

\subsection{Evaluation setup}
 
We follow an evaluation setup similar to Jain et al.~\citep{Jain15}. Algorithm~\ref{alg:inference} shows the inference steps for maneuver anticipation. At each time step $t$, features $\ve{x}_t$ and $\ve{z}_t$ are computed over the last 0.8 seconds of driving (20 frames). Using the temporal context $\{(\ve{x}_1,...,\ve{x}_t),\; (\ve{z}_1,...,\ve{z}_t)\}$, each anticipation algorithm computes the probability $\ve{y}_t$ for maneuvers in $ \mathcal{M} =$ \{\textit{left lane change, right lane change, left turn, right turn, driving straight}\}. The prediction threshold is denoted by $p_{th}\in(0,1]$ in Algorithm~\ref{alg:inference}. The algorithm predicts \textit{driving straight} if none of the softmax probabilities for the other maneuvers exceeds $p_{th}$.

%The prediction threshold $p_{th}$  reflects the confidence of an anticipation algorithm in its prediction. The algorithm predicts \textit{driving straight} if it is not atleast $p_{th}$ confident about its prediction in the remaining maneuvers. 

In order to evaluate an anticipation algorithm, we compute the following quantities for each maneuver $m \in \mathcal{M}$: (i) $N_m$: the total number of instances of maneuver $m$; (ii) $TP_m$: the number of instances of maneuver $m$ correctly predicted by the algorithm; and (iii) $P_m$: the number of times the algorithm predicts $m$. Based on these quantities we evaluate the  precision and recall of an anticipation algorithm as defined below: 

{\small \begin{align}
\label{eq:precision} Pr &= \frac{1}{|M|-1}\sum_{m \in \mathcal{M} \backslash \{\textit{driving straight}\}}\left(\frac{TP_m}{P_m}\right)\\
\label{eq:recall} Re &= \frac{1}{|M|-1}\sum_{m \in \mathcal{M} \backslash \{\textit{driving straight}\}}\left(\frac{TP_m}{N_m}\right)
\end{align}  }
We should note that  \textit{driving straight} maneuver is not included in evaluating  precision~\eqref{eq:precision} and recall~\eqref{eq:recall}. This is because anticipation algorithms by default predict \textit{driving straight} when they are not confident about other maneuvers.  For each anticipation algorithm, we choose a prediction threshold  $p_{th}$  that maximizes their $F1$ score: $F1 = 2*Pr*Re/(Pr+Re)$. In addition to precision and recall, we also measure the interval between the time an algorithm makes a prediction and the start of maneuver. We refer to this as the \textit{time-to-maneuver} and  denote it with $t_{before}$ in Algorithm~\ref{alg:inference}. We uniformly randomly partition the data set into five folds and report  results using 5-fold cross-validation. We train on four folds and test on the fifth fold, and report the metrics averaged over the five folds. 
%Prediction threshold $p_{th}$ allow anticipation algorithms to trade-off between precision and recall.

\begin{table*}[t!]
\centering
\caption{{\textbf{Maneuver Anticipation Results.} Average \textit{precision}, \textit{recall} and \textit{time-to-maneuver} are computed from 5-fold cross-validation. Standard error is also shown. Algorithms are compared on the features from Jain et al.~\citep{Jain15}.}}
\resizebox{1\textwidth}{!}{
\centering
\begin{tabular}{cr|ccc|ccc|ccc}
%\hline
&  &\multicolumn{3}{c}{Lane change}&\multicolumn{3}{|c}{Turns}&\multicolumn{3}{|c}{All maneuvers}\\
\cline{1-11}
\multicolumn{2}{c|}{\multirow{2}{*}{Method}} & \multirow{2}{*}{$Pr$ (\%)}  & \multirow{2}{*}{$Re$ (\%)} & Time-to-  & \multirow{2}{*}{$Pr$ (\%)} & \multirow{2}{*}{$Re$ (\%)} & Time-to-  & \multirow{2}{*}{$Pr$ (\%)} & \multirow{2}{*}{$Re$ (\%)}  & Time-to- \\ 
& & & &  maneuver (s) &  & &  maneuver (s) &  & & maneuver (s)\\\hline
&Chance	&	33.3		&	33.3		&	-	&	33.3		&	33.3		&	-	&	20.0		&	20.0		&	-\\
&SVM~\citep{Morris11}	&	73.7 $\pm$ 3.4	&	57.8 $\pm$ 2.8	&	2.40 		&	64.7 $\pm$ 6.5	&	47.2 $\pm$ 7.6	&	2.40 		&	43.7 $\pm$ 2.4	&	37.7 $\pm$ 1.8	& 1.20\\
&Random-Forest &   71.2 $\pm$ 2.4  &   53.4 $\pm$ 3.2  &   3.00    &   68.6 $\pm$ 3.5  & 44.4 $\pm$ 3.5  &   1.20      &   51.9 $\pm$ 1.6 &   27.7 $\pm$ 1.1  & 1.20\\
%Morris et al.~\citep{Morris11} RVM&&&&&&\\
%HMM $E$ & 75.0 (2.2) & 60.4 (5.7) & 3.46  &  74.4 (0.5) & 66.6 (3.0) & 4.04 & 63.9 (2.6) & 60.2 (4.2) & 3.26 \\
%HMM $F$		&	76.4 (1.4)	&	75.2 (1.6)	&	3.62		&	75.6 (2.7)	&		60.1 (1.7)	&	3.58 		&	64.2 (1.5)	&	36.8 (1.3)	&	2.61 \\
%HMM $E+F$	&	80.9 (0.9)	&	79.6 (1.3)	&	3.61 		&	73.5 (2.2)	&75.3 (3.1)	&	4.53 		&	67.8 (2.0)	&	67.7 (2.5)	&	3.72 \\
&IOHMM~\citep{Jain15}		&	81.6 $\pm$ 1.0	&	{79.6 $\pm$ 1.9}	&	3.98  	&	77.6 $\pm$ 3.3	&		{75.9 $\pm$ 2.5}	&	4.42 		&	74.2 $\pm$ 1.7	&	71.2 $\pm$ 1.6	&	3.83 \\
&AIO-HMM~\citep{Jain15}		&	{83.8 $\pm$ 1.3}	&	79.2 $\pm$ 2.9	&	3.80  		&	{80.8	 $\pm$ 3.4}	&		75.2 $\pm$ 2.4	&	4.16 		&	{77.4 $\pm$ 2.3}	&	{71.2 $\pm$ 1.3}	&	3.53 \\\hline
 & S-RNN & 85.4 $\pm$ 0.7 & 86.0 $\pm$ 1.4 & 3.53 & 75.2 $\pm$ 1.4 & 75.3 $\pm$ 2.1 & 3.68 & 78.0 $\pm$ 1.5 & 71.1 $\pm$ 1.0 & 3.15 \\
%(\textit{Our method}) SimpleRNN-decayingloss & 86.1 (0.02) & \textbf{89.6} (0.02) & 3.09 & 73.4 (0.01) & 72.3 (0.01) & 3.26 & 77.8 (0.03) & 75.3 (0.02) & 2.83 \\
\textit{Our}&F-RNN-UL & \textbf{92.7} $\pm$ 2.1 & 84.4 $\pm$ 2.8 & 3.46 & 81.2 $\pm$ 3.5 & 78.6 $\pm$ 2.8 & 3.94 & 82.2 $\pm$ 1.0 & 75.9 $\pm$ 1.5 & 3.75 \\
\textit{Methods}&F-RNN-EL & 88.2 $\pm$ 1.4 & \textbf{86.0} $\pm$ 0.7 & 3.42 & \textbf{83.8} $\pm$ 2.1 & \textbf{79.9} $\pm$ 3.5 & 3.78 & \textbf{84.5} $\pm$ 1.0 & \textbf{77.1} $\pm$ 1.3 & 3.58\\
%\hline
\end{tabular}
}
\label{tab:prscore}
\end{table*}

\begin{algorithm}[t]\caption{Maneuver anticipation}
\begin{algorithmic}
\STATE \textbf{Initialize} $m^* = \textit{driving straight}$\\
%$ \mathcal{M} =$ \{\textit{left lane change, right lane change, left turn, right turn, driving straight}\}
\STATE \textbf{Input} Features $\{(\ve{x}_1,...,\ve{x}_T),(\ve{z}_1,...,\ve{z}_T)\}$ and prediction threshold $p_{th}$
\STATE \textbf{Output} Predicted maneuver $m^*$
\WHILE{$t=1$ to $T$}
        \STATE Observe features $(\ve{x}_1,...,\ve{x}_t)$ and $(\ve{z}_1,...,\ve{z}_t)$
        \STATE Estimate probability $ \ve{y}_t$ of each maneuver in $\mathcal{M}$
        \STATE $m_t^*=\argmax_{m\in\mathcal{M}}\ve{y}_t$
		\IF{$m_t^* \neq \textit{driving straight}$ \& $\ve{y}_t\{m_t^*\} > p_{th} $}        
			\STATE $m^* = m_t^*$
			\STATE $t_{before} = T - t$
			\STATE \textbf{break}
		\ENDIF
        

\ENDWHILE
\STATE \textbf{Return} $m^*,t_{before}$
\end{algorithmic}
\label{alg:inference}
\end{algorithm}


\subsection{Results}

We evaluate anticipation algorithms on the maneuvers not seen during training with the following three prediction settings: (i) Lane change: algorithms only anticipate lane changes, i.e. $ \mathcal{M} =$ \{\textit{left lane change, right lane change, driving straight}\}. This setting is relevant for freeway driving; (ii) Turns: algorithms only anticipate turns, i.e. $ \mathcal{M} =$ \{\textit{left turn, right turn, driving straight}\}; and (iii) All maneuvers: algorithms anticipate all five maneuvers. Among these prediction settings, predicting all five maneuvers is the hardest. 

Table~\ref{tab:prscore} compares the performance of the baseline anticipation algorithms and the variants of our deep learning model. All algorithms in Table~\ref{tab:prscore} were evaluated on the features provided by Jain et al.~\citep{Jain15}, which ensures a fair comparison. We observe that variants of our architecture outperform the previous state-of-the-art a majority of the time. This improvement in performance is because RNNs with LSTM units are very expressive models, and unlike Jain et al.~\citep{Jain15} they do not make any assumption about the generative nature of the problem. 


The performance of several variants of our architecture, reported in Table~\ref{tab:prscore},  justifies our design decisions to reach the final architecture as discussed here.
%\noindent \textbf{How important is Fusion-RNN over Simple-RNN?} 
S-RNN performs a very simple fusion by concatenating the two sensor streams. On the other hand, F-RNN models each sensor stream with a separate RNN and then uses a fully connected layer at each time step to fuse the high-level representations. This form of sensory fusion is  more principled since the sensor streams represent different data modalities.  Fusing high-level representations instead of concatenating raw features gives a significant improvement in performance, as shown in Table~\ref{tab:prscore}.  When predicting all maneuvers, F-RNN-EL has a 6\%  higher precision and recall than S-RNN.







%\noindent \textbf{How useful is Exp-Loss over Uniform-Loss?}
As shown in Table~\ref{tab:prscore}, exponentially growing the loss improves performance. Our new loss scheme  penalizes the network proportional to the length of context it has seen.  When predicting all maneuvers, we observe that F-RNN-EL shows an improvement of 2\% in precision and recall over F-RNN-UL. We conjecture that exponentially growing the loss acts like a regularizer. It reduces the risk of our network over-fitting early in time when there is not enough context available. Furthermore, the time-to-maneuver remains comparable for F-RNN  with and without exponential loss. 



%\noindent \textbf{How informative are 3D head-pose features?} 
We study the effect of our improved features in Table~\ref{tab:features}. We replace the pipeline for extracting features from the driver's face~\citep{Jain15} by a Constrained Local Neural Field (CLNF) model~\citep{Baltrusaitis13}. Our new vision pipeline tracks 68 facial landmark points and estimates the driver's 3D head pose as described in Section~\ref{subsec:features}. 
%Table~\ref{tab:features} compares the performance of F-RNN-EL with these new features. 
We see a significant, 6\% increase in precision and 10\% increase in recall of F-RNN-EL when using features from our new vision pipeline. This increase in performance is attributed to the following reasons: (i) robustness of CLNF model to variations in illumination and head pose; (ii) 3D head-pose features are very informative for understanding the driver's intention; and (iii) optical flow trajectories generated by tracking facial landmark points represent head movements better, as shown in Figure~\ref{fig:feature_compare}.


\begin{table}[h]
\centering
\caption{\textbf{3D head-pose features.} In this table we study the effect of better features with best performing algorithm from Table~\ref{tab:prscore} in `All maneuvers' setting. We use~\citep{Baltrusaitis13} to track 68 facial landmark points and estimate 3D head-pose.}
{
\newcolumntype{P}[2]{>{\footnotesize#1\hspace{0pt}\arraybackslash}p{#2}}
\setlength{\tabcolsep}{2pt}
\centering
\resizebox{\hsize}{!}{
\begin{tabular}
{@{}p{0.40\linewidth}| P{\centering}{16mm}P{\centering}{16mm}P{\centering}{16mm}@{}}
%  &\multicolumn{3}{|c}{All maneuvers}\\
%\cline{2-10}
\multirow{2}{*}{Method} & \multirow{2}{*}{$Pr$ (\%)}  & \multirow{2}{*}{$Re$ (\%)} & Time-to-  \\ 
 & & &  maneuver (s)\\\hline
F-RNN-EL &  {84.5} $\pm$ 1.0 & {77.1} $\pm$ 1.3 & 3.58\\
%\hline
F-RNN-EL w/ 3D head-pose &  \textbf{90.5} $\pm$ 1.0 & \textbf{87.4} $\pm$ 0.5 & 3.16\\
\end{tabular}
}}
\label{tab:features}
\end{table}


\begin{figure*}[t]
\centering
\begin{subfigure}[b]{.23\textwidth}
	\includegraphics[width=\linewidth]{../Fig/confMat_rnn/SVM_I_O_precision.png}
	\caption{SVM~\citep{Morris11}}
	\end{subfigure}
\begin{subfigure}[b]{.23\textwidth}
	\includegraphics[width=\linewidth]{../Fig/confMat_rnn/AIOHMM_I_O_precision.png}
	\caption{AIO-HMM~\citep{Jain15}}
	\end{subfigure}	
	\begin{subfigure}[b]{.23\textwidth}
	\includegraphics[width=\linewidth]{../Fig/confMat_rnn/fusionrnn_old_features.png}
	\caption{F-RNN-EL}
	\end{subfigure}	
	\begin{subfigure}[b]{.23\textwidth}
	\includegraphics[width=\linewidth]{../Fig/confMat_rnn/fusionrnn_new_features.png}
	\caption{F-RNN-EL w/ 3D-pose}
	\end{subfigure}
	\caption{\textbf{Confusion matrix} of different algorithms when jointly predicting all the maneuvers. Predictions made by algorithms are represented by rows and actual maneuvers are represented by columns. Numbers on the diagonal represent precision.}
	\label{fig:confmat}	
\end{figure*}


\begin{figure}[t]
\centering
\includegraphics[width=0.8\linewidth]{../Fig/thresh_f1_rnn/thresh_f1.pdf}
\caption{\textbf{Effect of prediction threshold $p_{th}$.} At test time an algorithm makes a prediction only when it is at least $p_{th}$ confident in its prediction. This plot shows how F1-score vary with change in prediction threshold.}
\label{fig:f1score}
\end{figure}


The confusion matrix in Figure~\ref{fig:confmat} shows the precision for each maneuver. F-RNN-EL gives a higher precision than AIO-HMM on every maneuver when both algorithms are trained on same features (Fig.~\ref{fig:confmat}c). Our new vision pipeline further improves the precision of F-RNN-EL on all maneuvers (Fig.~\ref{fig:confmat}d). Additionally, both F-RNN and AIO-HMM perform significantly better than previous work on maneuver anticipation by Morris et al.~\citep{Morris11} (Fig.~\ref{fig:confmat}a).


%\noindent \textbf{What is the effect of prediction threshold $p_{th}$?} 
In Figure~\ref{fig:f1score} we study how F1-score varies as we change the prediction threshold $p_{th}$.  We make the following observations: (i) The F1-score does not undergo large variations with changes to the prediction threshold. Hence, it allows practitioners  to fairly trade-off between the precision and recall without hurting the F1-score by much; and (ii)   the maximum F1-score attained by F-RNN-EL is 4\% more than AIO-HMM when compared on the same features and 13\% more with our new vision pipeline.
In {Tables~\ref{tab:prscore} and \ref{tab:features}}, we used the threshold values which gave the highest F1-score.
\iffalse
In summary, our deep learning approach significantly improves the state-of-the-art in maneuver anticipation. Inference in our architecture is a simple forward-pass which happens in real-time using dynamic programming. Our approach to maneuver anticipation is directly applicable to industrial efforts on driver intention prediction and anticipation~\citep{BoschURBAN}.
\fi

\iffalse
We also analyze the performance when the anticipation algorithms make predictions at a fixed time interval before the maneuver, as shown in Figure~\ref{fig:ttm}.
%shows how F1-score varies when . 
This prediction strategy is different from Algorithm~\ref{alg:inference},  where an anticipation algorithm makes a prediction when it is most confident about the maneuver. We observe that the F1-score increases (not strictly) as we move closer to the instant when the maneuver happens. This shows that more context enables anticipation algorithms to make better predictions. In practice we use the prediction strategy described in Algorithm~\ref{alg:inference}, since the instant when the maneuver occurs is not known in advance. 	



\begin{figure}[t]
\vspace{-0.05in}
\centering
\includegraphics[width=0.8\linewidth]{../Fig/time_prediction/time_predict_rnn.pdf}
\vspace{0.9\captionReduceTop}
\caption{\textbf{Effect of time-to-maneuver.} Plot shows how F1-score vary as algorithms predict at a fixed time before the maneuver happens.}
\vspace{1.2\captionReduceBot}
\label{fig:ttm}
\end{figure}
\fi


==> intro_backup.tex <==

% !TEX root = main.tex
\section{Introduction}
Over the last decade
cars have been equipped with various assistive technologies in order to
provide a safe driving experience. Technologies such as lane keeping, blind spot check,
pre-crash systems etc.,  are successful in alerting drivers whenever they commit a
dangerous maneuver~\citep{Laugier11}. Still in the US alone more than 33,000 people die in road
accidents every year, the majority of which are due to inappropriate
maneuvers~\cite{road_accidents}. 
We need mechanisms that	 can alert drivers \textit{before} they perform a dangerous maneuver 
in order to avert many such accidents~\citep{Rueda04}.  
In this work we address this problem of anticipating maneuvers that a
driver is likely to perform in the next few seconds (Figure~\ref{fig:intro}). 
%We use
%various cues from inside and outside of the vehicle (Figure~\ref{fig:intro}), and 
%present a learning algorithm for reasoning about the future maneuvers.

Anticipating the future actions of a human is an important perception task and has many applications in robotics and computer vision~\citep{Kuderer12,Ziebart09,Kitani12,Koppula13,Wang13}. Figure~\ref{fig:intro} 
shows our system anticipating a left turn maneuver a few seconds before the car reaches the 
intersection. Our system also outputs probabilities over the  maneuvers the driver can perform. 
With this prior knowledge of maneuvers, the driver assistance systems can 
alert drivers about possible dangers before they perform the maneuver, 
thereby giving them more time to react. Some previous works~\citep{Frohlich14,Kumar13,Morris11} also predict a driver's  future maneuver.  However, as we show in the following sections, these methods use limited context and do not accurately model the anticipation problem.

\begin{figure}[t]
\centering
\includegraphics[width=.8\linewidth]{../Fig/intropic/intropic.pdf}
\caption{\textbf{Anticipating maneuvers.} Our algorithm anticipates driving maneuvers performed a few seconds in the future. It uses information from multiple sources including videos, vehicle dynamics, GPS, and street maps to anticipate the probability of different future maneuvers.}
\label{fig:intro}
\end{figure}


In order to anticipate maneuvers, we reason with the contextual information from 
the surrounding events, which we refer to as the \textit{driving context}. % as well as from inside the vehicle. 
We obtain this driving context from multiple sources. We use videos
of the driver inside the car and the road in front, the vehicle's dynamics,
global position coordinates (GPS), and street maps; from this we extract a
time series of multi-modal data from both inside and outside the vehicle. The
challenge lies in modeling the temporal aspects of driving and in detecting the contextual
cues that help in anticipating maneuvers.
%It further requires joint reasoning of the driving context and the driver's intention. The challenge here is the driver's intentions are not directly observable, and their interactions with the driving context are complex. For example, the driver is influenced by external events such as traffic conditions. 
Hence we propose a specially tailored modeling approach for anticipation in such sensory-rich settings.

Modeling anticipation is challenging because it requires the prediction of future events from  a limited temporal context. It is different from \textit{activity recognition}~\citep{Wang13}, where the complete temporal context is available for prediction.  Furthermore, in sensory-rich robotics settings like ours, the context for anticipation comes from multiple sensors. In such scenarios the end performance of the application largely depends on how the information from different sensors are fused. Previous works on anticipation~\citep{Kitani12,Koppula13,Kuderer12} usually deal with single-data modality and do not address anticipation for sensory-rich robotics applications. Additionally, they learn representations using shallow architectures~\citep{Jain15,Kitani12,Koppula13,Kuderer12} that cannot handle long temporal dependencies~\citep{Bengio11}. 

\begin{figure}[t]
\centering	
\includegraphics[width=\linewidth]{../Fig/rnn_b4c/rnn_anticipation.pdf}
\caption{(\textbf{Left}) Shows training RNN for anticipation in a sequence-to-sequence prediction manner. The network explicitly learns to map the partial context $(\ve{x}_1,..,\ve{x}_t)\;\forall t$ to the future event $\ve{y}$. (\textbf{Right}) At test time the network's goal is to anticipate the future event as soon as possible, i.e. by observing only a partial temporal context.}
\label{fig:introfig}
\end{figure}

In order to address the anticipation problem more generally, we propose a Recurrent Neural Network (RNN) based architecture which learns rich representations for anticipation. We focus on sensory-rich robotics applications, and our  architecture learns how to optimally fuse information from different sensors. Our approach  captures temporal dependencies by using Long Short-Term Memory (LSTM) units.  We train our architecture in a sequence-to-sequence prediction manner (Figure~\ref{fig:introfig}) such that it explicitly learns to anticipate given a partial context, and we introduce a novel loss layer which helps anticipation by preventing over-fitting. 

We evaluate our approach on a driving data set with 1180 miles of natural freeway and
city driving collected across two states -- from 10 drivers and with different kinds of driving maneuvers. The data set is challenging because of the variations in routes and traffic conditions, and the driving styles of the drivers (Figure~\ref{fig:dataset}). We demonstrate that our deep learning sensory-fusion approach anticipates 
maneuvers 3.5 seconds before they occur with {84.5\%} precision and {77.1\%} recall while using out-of-the-box face tracker. With more sophesticated 3D pose estimation of the face, our precision and recall increases to \textbf{90.5\%} and \textbf{87.4\%} respectively. We believe that our work creates scope for new ADAS features to make roads safer. In summary our key contributions are as follows: 


 \begin{figure}[t]
\centering	
\includegraphics[width=.9\linewidth]{../Fig/rnn_b4c/dataset.pdf}
\caption{\textbf{Variations in the data set.} {Images from the data set~\citep{Jain15} for} a left lane change. (\textbf{Left}) Views from the road facing camera. (\textbf{Right}) Driving style of the drivers vary for the same maneuver.}
\label{fig:dataset}
\end{figure}

\begin{itemize}
\itemsep0em 
\item We propose a sensory-rich approach for anticipating driving maneuvers several seconds in advance.
\item A sensory-fusion RNN-LSTM architecture for anticipation in sensory-rich robotics applications.
\item We release the first data set of natural driving with videos from both inside and outside the car, GPS, and speed information.
\item We release an open-source deep learning package \href{https://github.com/asheshjain399/NeuralModels}{\texttt{NeuralModels}} which is especially designed for robotics applications with multiple sensory streams. 
\end{itemize}
Our data set and deep learning code are publicly available at: \url{http://www.brain4cars.com}

==> maneuver_backup.tex <==
% !TEX root = main.tex

\section{Training the network for maneuver anticipation}
\label{sec:maneuver}
In maneuver anticipation the goal is to anticipate the driver's future maneuver several seconds before it happens~\citep{Jain15,Morris11}. The contextual information for anticipation is extracted from sensors installed in the vehicle. Previous work from Jain et al.~\citep{Jain15} consider the context from a driver facing camera, a camera facing the road in front, a Global Positioning System (GPS), and an equipment for recording the vehicle's dynamics. The overall contextual information from the sensors is grouped into: (i) the context from inside the vehicle, which comes from the driver facing camera and is represented as temporal sequence of features $(\ve{x}_1,...,\ve{x}_T)$; and (ii) the context from outside the vehicle, which comes from remaining sensors and is represented as $(\ve{z}_1,...,\ve{z}_T)$.

 In order to anticipate maneuvers our RNN architecture (Figure~\ref{fig:fusion}) processes temporal context $(\ve{x}_1,...,\ve{x}_t)$ and $ (\ve{z}_1,...,\ve{z}_t)$  at every time step $t$, and outputs softmax probabilities $\ve{y}_t$ for the following five maneuvers:  $\mathcal{M}=$~\{\textit{left turn}, \textit{right turn}, \textit{left lane change}, \textit{right lane change}, \textit{straight driving}\}. We now give an overview of our feature representation and then describe our training procedure.



\iffalse
In maneuver anticipation the goal is to anticipate a vehicle's future maneuver several seconds before it happens~\citep{Jain15,Morris11}. The contextual information for anticipation is extracted from sensors installed in the vehicle. Previous work from Jain et al.~\citep{Jain15} and Morris et al.~\citep{Morris11} consider the context comprising of two sensory streams: (i) $(\ve{x}_1,...,\ve{x}_T)$ represents the driving context inside the vehicle such as the driver's head movements; and (ii) $(\ve{z}_1,...,\ve{z}_T)$ represents the driving context outside the vehicle such as lane or traffic information.
In order to anticipate maneuvers our RNN architecture (Figure~\ref{fig:fusion}) processes temporal context $(\ve{x}_1,...,\ve{x}_t)$ and $ (\ve{z}_1,...,\ve{z}_t)$  at every time step $t$, and outputs softmax probabilities $\ve{y}_t$ for the following five maneuvers:  $\mathcal{M}=$~\{\textit{left turn}, \textit{right turn}, \textit{left lane change}, \textit{right lane change}, \textit{straight driving}\}. We now describe our training procedure and give an overview of our feature representation.
\fi

\begin{figure*}[t]
\centering	
\includegraphics[width=\linewidth]{../Fig/rnn_b4c/sys_fig.png}
\caption{\textbf{Maneuver anticipation pipeline.} Temporal context in maneuver anticipation comes from cameras facing the driver and the road, GPS, and the vehicle's dynamics. (\textbf{a}, \textbf{b} and \textbf{c}) We improve upon the vision pipeline from Jain et al.~\citep{Jain15} by tracking 68 landmark points on the driver's face and including 3D head-pose features. (\textbf{d}) Using Fusion-RNN we combine the sensory streams of features from inside the vehicle (driver facing camera) and outside the vehicle (road camera, GPS, vehicle dynamics).}
\end{figure*}


\subsection{Features}
\label{subsec:features}
\iffalse
We give an overview of the vehicle setup and feature representation from Jain et al.~\citep{Jain15} and describe our feature improvements. The vehicle for maneuver anticipation is equipped with a driver facing camera, a camera facing the road in front, a Global Positioning System (GPS), and an equipment for recording the vehicle's dynamics. The overall contextual information from the sensors is grouped into: (i) the context from inside the vehicle, which comes from the driver facing camera and is represented as temporal sequence of features $(\ve{x}_1,...,\ve{x}_T)$; and (ii) the context from outside the vehicle,  which comes from remaining sensors and is represented as $(\ve{z}_1,...,\ve{z}_T)$.
\fi

We now describe the feature representation of $\ve{x}_t$ and $\ve{z}_t$ from Jain et al.~\citep{Jain15}.
The driver facing camera detects discriminative points on the driver's face and tracks the detected points across frames using KLT tracker~\citep{Shi94}. The tracking generates 2D optical flow trajectories in the plane of image. From these trajectories the horizontal and angular movements of the face are extracted, and these movements are binned into histogram features for every frame. These histogram features are aggregated over 20 frames (i.e. 0.8 seconds of driving) and constitute the feature vector  $\ve{x}_t \in \mathbb{R}^9$. 
Further context for anticipation comes from the camera facing the road, the GPS, 
and the vehicle's dynamics. This is denoted by the feature vector $\ve{z}_t \in \mathbb{R}^6$, and includes the lane information, the road artifacts such as intersections, and the vehicle's speed. 
We refer the reader to Jain et al.~\citep{Jain15} for more information.

\textbf{3D head pose and facial landmark features.} We propose improvements over the features from Jain et al.~\citep{Jain15}. Instead of tracking discriminative points on the driver's face we use Active Appearance Model (AAM)~\citep{Cootes01} and track 68 fixed  landmark points on the driver's face~\citep{Baltrusaitis13}. This offers us two distinct benefits: (i) while discriminative facial points may change from situation to situation, tracking fixed landmarks results in consistent optical flow trajectories; and (ii) it also allows us to estimate 3D head pose of the driver's face by minimizing the error in projection of a generic 3D mesh model of the face w.r.t. the 2D location of landmarks in the image. Including 3D head pose features (yaw, pitch, and roll) with the histogram features generated from optical flow trajectories gives $\ve{x}_t \in \mathbb{R}^{12}$. 

In Section~\ref{experiments} we present results with the features from Jain et al.~\citep{Jain15}, as well as the results with our improved AAM features.

\iffalse
\subsection{Data augmentation and model training}
\label{subsec:augmentation}

Before training our network for maneuver anticipation we add redundancy to the training data by data augmentation. The redundant data acts like a regularizer and reduces the risk of over fitting~\citep{Krizhevsky12,Hannun14}. 
%Data augmentation has been shown to work well on image and speech recognition tasks~\citep{Krizhevsky12,Hannun14}. 
While data augmentation has been well studied for feed-forward networks such as Convolutional Neural Networks~\citep{Krizhevsky12}, it is not yet clear how to augment data for RNNs. We augment data for maneuver anticipation by extracting sub-sequences of temporal context. Given a training example with two temporal sensor streams $\{(\ve{x}_1,...,\ve{x}_T),(\ve{z}_1,...,\ve{z}_T),y\}$, we uniformly randomly sample multiple sub-sequences $\{(\ve{x}_i,...,\ve{x}_j),(\ve{z}_i,...,\ve{z}_j),y | 1 \leq i < j \leq T\}$ as additional training examples. It is important to realize that data augmentation only adds redundancy and does not rely on any external source of new information. 
\iffalse
Data augmentation involves increasing the size of training data by adding new examples that are either synthetically generated, or obtained through various \textit{augmentation} operations on the training data set. Since the number of parameters in a deep network is typically more than the number of training examples, data augmentation reduces the risk of over fitting. It has been shown to work well on image and speech recognition tasks~\citep{Krizhevsky12,Hannun14}. While data augmentation has been well studied for feed-forward networks such as Convolutional Neural Networks~\citep{Krizhevsky12}, it is not yet clear how to augment data for RNNs.  In order to train our network for maneuver anticipation we augment the training data by extracting sub-sequences of temporal context. Given a training example with two temporal sensor streams $\{(\ve{x}_1,...,\ve{x}_T),(\ve{z}_1,...,\ve{z}_T),y\}$, we uniformly randomly sample multiple sub-sequences $\{(\ve{x}_i,...,\ve{x}_j),(\ve{z}_i,...,\ve{z}_j),y | 1 \leq i < j \leq T\}$ as additional training examples.	
\fi

On the augmented data set we train the network described in Section~\ref{sec:sensor-fusion-rnn}. We use RMSprop gradients which have been shown to work well on training deep networks~\citep{Dauphin15}, and we keep the step size fixed at $1e^{-4}$. We experimented with different variants of softmax loss, however, our proposed loss-layer with exponential growth Eq.~\eqref{eq:loss} works best for anticipation (see Section~\ref{experiments} for details).
\fi


\iffalse
We use Stochastic Gradient Descent (SGD)~\citep{Bottou10} to minimize the exponentially growing loss function. We use RMSprop gradients in SGD which has been shown to work well on training deep networks~\citep{Dauphin15}, and we keep the step size fixed at $1e^{-4}$. We experimented with different variants of softmax loss, however, our proposed loss-layer with exponential decay~\eqref{eq:loss} works best for anticipation. See Section~\ref{experiments} for details.
\todo{move equation~\eqref{eq:loss} to the para describing the loss?}
\fi

